Compact recurrent neural networks for acoustic event detection on low-energy low-complexity platforms

Outdoor acoustic events detection is an exciting research field but challenged by the need for complex algorithms and deep learning techniques, typically requiring many computational, memory, and energy resources. This challenge discourages IoT implementation, where an efficient use of resources is required. However, current embedded technologies and microcontrollers have increased their capabilities without penalizing energy efficiency. This paper addresses the application of sound event detection at the edge, by optimizing deep learning techniques on resource-constrained embedded platforms for the IoT. The contribution is two-fold: firstly, a two-stage student-teacher approach is presented to make state-of-the-art neural networks for sound event detection fit on current microcontrollers; secondly, we test our approach on an ARM Cortex M4, particularly focusing on issues related to 8-bits quantization. Our embedded implementation can achieve 68% accuracy in recognition on Urbansound8k, not far from state-of-the-art performance, with an inference time of 125 ms for each second of the audio stream, and power consumption of 5.5 mW in just 34.3 kB of RAM.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> comments.tex <==
%% bare_conf.tex
%% V1.4b
%% 2015/08/26
%% by Michael Shell
%% See:
%% http://www.michaelshell.org/
%% for current contact information.
%%
%% This is a skeleton file demonstrating the use of IEEEtran.cls
%% (requires IEEEtran.cls version 1.8b or later) with an IEEE
%% conference paper.
%%
%% Support sites:
%% http://www.michaelshell.org/tex/ieeetran/
%% http://www.ctan.org/pkg/ieeetran
%% and
%% http://www.ieee.org/


%%*************************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE! 
%% User assumes all risk.
%% In no event shall the IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%
%% This work is distributed under the LaTeX Project Public License (LPPL)
%% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
%% distributed and modified. A copy of the LPPL, version 1.3, is included
%% in the base LaTeX documentation of all distributions of LaTeX released
%% 2003/12/01 or later.
%% Retain all contribution notices and credits.
%% ** Modified files should be clearly indicated as such, including  **
%% ** renaming them and changing author support contact information. **
%%*************************************************************************

% *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% *** with production work. The IEEE's font choices and paper sizes can   ***
% *** trigger bugs that do not appear when using other class files.       ***                          ***
% The testflow support page is at:
% http://www.michaelshell.org/tex/testflow/

% Some Computer Society conferences also require the compsoc mode option,
% but others use the standard conference format.
%
% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[conference]{../sty/IEEEtran}





% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)


% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%
%\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.






% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.




% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix




% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.




% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )



==> experimental_analisys.tex <==
\section{Experimental Analysis}
\label{sec:experiments}
Considering \ac{SED} in outdoor urban environments, two datasets are often used in literature: \textit{UrbanSound8K} and TUT Sound events 2017. The latter is particularly attractive because it features real recordings and several comparative methods are available thanks to the related challenge DCASE2017 \cite{DCASE2017challenge}. Unfortunately, the task is very challenging and classes are highly unbalanced, preventing a fair evaluation of \ac{KD} methods. %Therefore, we used \textit{UrbanSound8K}, altought 
%The latter target sound event classes were selected to represent common sounds related to human presence and traffic. Unfortunately, classes are strongly imbalanced, so \ac{KD} transfers to the student only capability to classify frequent events. For this reason, we focused on , where classes are balanced.

Therefore, %for our experimental analysis
we used the \textit{UrbanSound8K} dataset \cite{salamon2014dataset}. It includes 8732 audio samples related to the city environment, with different sampling rates, number of channels and maximum length of 4 seconds. Each recording has a unique label among ten possible classes: air conditioner, car horn, children playing, dog bark, drilling, engine idling, gun shot, jackhammer, siren, and street music. 
%An additional salience description indicates whether the occurrence are subjectively perceived to be in the foreground or background of the recording. 
All clips are taken from Freesound\footnote{"http://www.freesound.org"}, a huge collaborative database of audio samples.

Following the recipe reported in \cite{salamon2014dataset}, we use 10-fold cross validation and average scores. %Thus, each of the 10 folds is used for test and the remaining 9 for training. 
However, we took one additional fold for validation: 8 folds are used as training data, one is used as validation and the remaining one for test (training-validation-test ratio is 0.8-0.1-0.1). Performance is measured in terms of classification accuracy. In some experiments, the dataset is augmented through pitch shifting \cite{salamon2017deep}, with both positive (up) and negative (down) semitones with values {-2,-1,1,2}.

\subsection{Teacher}
State-of-the-art solutions for \ac{SED} are mostly \ac{CNN} fed with mel-spectrogram \cite{piczak2015environmental}\cite{zhang2018deep}\cite{zhang2017dilated}. However, to fully exploit the potential of the~\ac{KD} approach, rather than training from scratch our big \ac{CNN}, we employed the publicly available VGGish\footnote{"https://github.com/tensorflow/models/tree/master/research/audioset"} feature extractor~\cite{hershey2017cnn}, followed by a classification stage tailored on \textit{UrbanSound8K}. VGGish is trained on the Youtube-8M Dataset \cite{gemmeke2017audio} and it is expected to generalize well to other application contexts. Note that this fact introduces a further novelty in our work since distillation is performed on a different dataset than that used in the original training. %In this work, we mimic a feature extractor trained on a Dataset to make it extract meaningful embedded on another Dataset (Urbansound8k). This approach is novel and let the student classifier to be less complicated, because tailored to the specific task, instead of being generic for every sound.
VGGish converts \SI{960}{\milli\second} audio input mel spectrogram into a 128 dimensional embedding that can be used as input for a further classification model. The classifier can be shallow as the VGGish embeddings are more semantically compact (than raw audio features). The VGGish architecture is described in Table \ref{tab:models}. For all the convolutional layers the kernel size is 3, the stride is 1 and the activation function is ReLu. Max pooling layers are implemented with a 2x2 kernel and a stride of 2.

The classifier consists of a \ac{GRU} followed by a fully connected layers and maps the VGGish embeddings into the 10 classes of \textit{UrbanSound8K}. A BatchNormalization layer is inserted between the feature extractor and the classifier to accelerate training. 

VGGish expects as input \SI{960}{\milli\second} of audio signal sampled at \SI{16}{\kilo\hertz}. Each clip in \textit{UrbanSound8K} is resampled and padded or cropped to get a length of 960*4=\SI{3840}{\milli\second}. The resulting signal is divided into 4 non-overlapping \SI{960}{\milli\second} frames. For each frame, the short-time Fourier transform is computed on \SI{25}{\milli\second} windows every \SI{10}{\milli\second}. The resulting spectrogram is integrated into 64 mel-spaced frequency bins, covering the range 125-7500 Hz, and log-transformed. This gives 4 patches of 96 x 64 bins that form the input of the VGGish.


\subsection{Student}

Although our goal is to fit the classifier on an \ac{IoT} device, we consider 4 different degrees of compression, to better assess the potential and limits of the proposed approach.
Note that the student networks reduce drastically the feature extractor only. The classifier is re-trained, but it keeps the same architecture, i.e. a recurrent layer and 10-unit fully connected layers. 
We evaluate 4 training strategy based on the 4 losses in section \ref{sec:knowledgedistillation}. Weights are listed in Table \ref{tab:alphas}. The $T_{e}$ training procedure is composed by two independent training stages: the student is trained to replicate the VGGish features, minimizing the cost function in eq.\ref{eq:emb}; then the classifier is trained with the hard loss in equation \ref{eq:hardLoss}). For each training strategy we train 5 different models. 
\begin{table}[th]
  \caption{Combination weights for different training strategies}
  \label{tab:alphas}
  \centering
\begin{tabular}{l|ccc}
            & $\alpha_{h}$  & $\alpha_{s}$  & $\alpha_{e}$  \\ \hline
$T_h$       & 1             & 0             & 0             \\
$T_{h,s}$   & 0.5           & 1             & 0             \\
$T_{h,s,e}$ & 1             & 1             & 1             \\
$T_{e} $    & 0             & 0             & 1             
\end{tabular}
\vspace{-0.3cm}
\end{table}

Table \ref{tab:models} shows the different network, built changing layers and number of filters in an heuristic way. The model subscript is the approximate number of parameter of the upstream part.
\begin{figure*}[th]
  \centering
  \includegraphics[width=0.8\textwidth]{Accuracy_For_Different_training_procedure.png}
  \caption{Average accuracy for the 5 different models in table \ref{tab:models} with (right) and without (left) data augmentation. Each line represents a different training strategy. Dashed line is the teacher accuracy.}
  \label{fig:accuracyVsTraining}
  \vspace{-0.4cm}
\end{figure*}
%All the network, except M$_{20k}$, uses padding in convolutional layer. 
\begin{table}[th]
  \caption{Architecture of the models under analysis. "-" means that the layer is not active, "x" means that the layer is active.}
  \label{tab:models}
  \centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
Layer & VGGish & M$_{20M}$  & M$_{2M}$ & M$_{200k}$ & M$_{20k}$\\ \hline
Conv1 & 64      & 64 & 32  & 8    & 4   \\
Pool1 & x       & x  & x   & x    & x   \\
Conv2 & 128     &128 & 64  & 16   & 8   \\
Pool2 & x       & x  & x   & x    & x   \\
Conv3 & 256     &256 & 128 & 32   & 16  \\
Conv4 & 256     & -  & -   & -    & -   \\
Pool3 & x       & x   & x & x    & x    \\
Conv5 & 512     &256  & 128 & 64   & 16 \\
Conv6 & 512     & -     & -   & -    & -\\
Pool4 & x       & x & x   & x    & x   \\
Conv7 & -       & - & -   & 64   & 32  \\
Pool5 & -       & - & -   & x    & x   \\
FC1   & 4096    & 2048 & 512 & 256  & 64\\
FC1   & 4096    & 2048 & -   & -    & - \\
FC2   & 128     & 128 & 128 & 128  & 128\\
BatchNorm & x   & x & x  &  x   &  x    \\
GRU   & 20      & 20 & 20  & 20   & 20  \\
FC3   & 10      & 10 & 10  & 10   & 10 
\end{tabular}
}
\vspace{-0.3cm}
\end{table}
%
\begin{table}[ht]
  \caption{Computational and memory requirements for each network}
  \label{tab:models_costs}
  \centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
  & VGGish & M$_{20M}$  & M$_{2M}$ & M$_{200k}$ & M$_{20k}$\\ \hline
\#Param & \ti72.1M & \ti18.0M & \ti1.88M & \ti202k & \ti30.6k \\
\#Ops & \ti1.72G & \ti608M & \ti148M& \ti13.6M & \ti2.11M \\
\#Buffer & \ti614k & \ti602k & \ti301k & \ti76.0k & \ti 34.3k 
\end{tabular}
}\vspace{-0.4cm}
\end{table}
Table~\ref{tab:models_costs} reports the computational requirements of each network: number of parameter to store, operations and buffer size.
This approximation refers to an implementation using 8-bit quantized weights and buffers size as specified in the CMSIS-NN library, an embedded-C framework for neural network developed for Cortex M4-M7 based microcontroller\cite{lai2018cmsis}. During training is important to have floating-point 32-bit representation, because it allows fine tuning. However, such high precision is not required during inference \cite{lin2016fixed}.
With 8 bit quantization assumption, each parameter takes one byte, thus the number of parameters is equal to the non-volatile memory needed.

The number of operations (both multiplications and sums) depends on the layer type: in convolution and maxpooling layers, each output pixel comes from a filter application, then each filter application requires, given the kernel size $k$ and the number of input channels $c$:
\begin{align}
Ops_{filter} &= 2\cdot c\cdot k^2 \\
Ops_{Conv} &= Ops_{filter} \cdot out_{H} \cdot out_{W} \cdot out_{C}
\end{align}
%the 2 comes because of both sum and multiplication. 
%The same is for max pooling.

For dense and \ac{GRU} layers the number of operations is the number of matrix multiplications:
\begin{equation}
Ops_{DotProduct} = 2\cdot in_{shape} \cdot out_{shape} 
\end{equation}
%In dense layers, the number of operations is exactly the operation of matrix dot product. For \ac{GRU} the dot product is applied three times.
Gated recurrent unit requires also small element-wise product.

Concerning the buffer size, one buffer must contain the biggest input of all layers and another one must contain the biggest output, because they can be reused in following layers.


==> related_works_old.tex <==
\section{Related Works} \label{sec:relatedwork}
Nowadays, deep neural networks are the state-of-the-art for many classification tasks like image classification, speech recognition and so on. The trend is to use networks of continuously increasing size and complexity, motivated by the fact that they  generalize better than shallower ones~\cite{canziani2016analysis}. As a consequence, the most recent and advanced solutions may be not practical if limited computational resources are available, as in the case of IoT application contexts. However, in those IoT-related scenarios, reducing the network complexity and preserving as much as possible of its generalization capability is of major interest. % perchè? finirei la frase  con un ... to enable energy-efficient oppure taglio quanto segue e metto In fact... 
%qui il passaggio a quanto segue non è chiaro, si parla all'improvviso di SED... metterei qui reference a lavori che provano l'interesse di andare at the edge...
%Low power consumption and scalability of \ac{IoT} systems make microcontrollers an obvious choice for deploying \ac{SED}. 
%i nodi IoT per essere efficienti devono avere hardware efficiente e fortunatamente c'è... microcontorllore
%Microcontrollers are low-cost energy-efficient processing units and nowadays their computation capability allows non-trivial processing on board; but still, these systems have some severe constraints in terms of limited memory footprint (up to hundreds of \si{\kilo\byte}) and limited computation resources. 

In fact, \ac{IoT} nodes can be used as simple sensing devices, transmitting all the information directly to the cloud (\cite{kelly2013towards, piyare2017plug}). Nevertheless, this transmission is usually expensive from an energy point of view, thus, processing data locally on the node can be preferred, especially when the throughput is considerably high (audio, inertial movement unit, video and so on). 
%
%With this in mind, processing on-board is indispensable to extract meaningful information from the data, like classification \cite{paissan2019}. 
%
{\color{red} Fortunately, technology comes in to help,} since the microcontrollers available nowadays are low-cost, energy-efficient processing units with average computation capability that allows non-trivial processing on board; nevertheless, these systems have some severe constraints, for example in terms of limited memory footprint (up to hundreds of \si{\kilo\byte}). %and limited computation resources.

Enabling advanced machine learning in \ac{IoT} nodes is therefore of great interest and is becoming an attractive research topic {\color{red} for a variety of digital signal processing applications.}%, for example in computer vision. 


%[secondo me qui come primo lavoro di esempio non ci può essere il nostro...] 

{\color{red} One way to achieve edge deep learning is employing non-commercial platforms optimized for neural networks. As an example, in~\cite{palossi2018ultra} an ultra-low power deep-learning-powered autonomous nano-drone using a dedicated processing platform with state-of-the-art energy efficiency is used. In this way, no particular efforts are required in the network design thanks to the capabilities of the device. Processing time and memory footprint are further reduced by properly quantizing the network. Quantization is also relevant in \cite{cerutti2019convolutional} where, in combination with the use of the CMSIS-NN library, an embedded-C framework for neural network developed for Cortex M4-M7 based microcontrollers \cite{lai2018cmsis}, it allows a very quick and low-power classification of  thermal images. However, the neural architecture is rather small (three-layer \ac{CNN}) and the resolution of the thermal images is very low (8x8).}
%Data from a thermopile sensor enables real-time people detection in \cite{cerutti2019convolutional}. The microcontroller processes frame by frame the thermal map generated from the sensor through a three-layer \ac{CNN}. Each classification takes 3 ms and consumes only 30 \si{\milli\watt}. These results come from the combination of the network quantization and the use of the CMSIS-NN library, an embedded-C framework for neural network developed for Cortex M4-M7 based microcontrollers \cite{lai2018cmsis}.
%On the other hand, the thermal images have a very low resolution (8x8); thus, the processing of such data (64) is not as time-consuming as standard image classification. 
%Other researches explore the use of non-commercial platforms optimized for neural networks ~\cite{palossi2018ultra}. They designed an ultra-low power deep-learning-powered autonomous nano-drone using a dedicated processing platform with state-of-the-art energy efficiency. Authors use quantization to reduce footprint and processing time, while no other compression techniques like network pruning or knowledge distillation are explored. 

{\color{red} The previous examples do not tackle the porting of deep learning on micro-controllers from an algorithmic point of view, because either the device is very powerful or the feature dimensionality is very small. The improvement obtained via quantization is somehow "imposed" by the fixed point representation of the micro-controller. However, for other classification tasks, in particular those involving the processing of audio streams, the approaches presented above are not practicable as very large neural networks as well as feature vectors are employed in state-of-the-art solutions.}

%{\color{red} The previous examples show the scientific interest in the domain of computer vision regarding the possibility of bringing high-end computation, such as CNN to low-end resource-constrained devices. A similar trend happens with audio signal processing. Keyword spotting is a typical problem in speech recognition requiring a near-to-the speaker always-on smart device, thus calling for an energy-efficient embedded system with on-board recognition capabilities optimized for the purpose.}


%Keyword spotting is another field of interest where low power systems are required because devices must be always-on and embedded in battery-powered smart-devices.
%To ensure the best user experience, the keyword spotter should detect the keywords with high accuracy and low latency.
{\color{red} In keyword spotting, which requires near-to-the speaker always-on smart devices and thus calling for an energy-efficient embedded system with on-board recognition capabilities optimized for the purpose, a common strategy is designing and implementing small networks, specifically fitted to the hardware capacity, that can be trained from scratch and ported on low-power low-cost microcontrollers. }Authors of \cite{Sainat2015cnnkws} show the improvement of convolutional neural networks compared to standard deep neural networks in terms of performance, number of parameters and operations. Tang et Al. \cite{Tang2018residual} implemented a set of residual neural networks with specific compact structures, focused on reducing the overall number of parameters and operations. 
%Both these works do not give any reference regarding a real implementation on keyword spotting. 
Zhang et Al. \cite{zhang2017hello} implemented a keyword spotting on a commercial microcontroller platform using fixed-point quantization and CMSIS-NN implementation of deep neural networks. The inference time is around \SI{12}{\milli\second}; thus, it gives a responsive user experience. Unfortunately, they do not provide any consumption measurement of their system.


%The methods described above focus on designing and implementing small networks that can be trained from scratch and ported on low-power low-cost microcontrollers. 

A completely different strategy is to compress an existing model, generating a new network with smaller memory footprint but that effectively mimics the original one. In literature, several approaches exist to reduce the number of parameters of a neural network. Network pruning \cite{hassibi1993optimal} aims at detecting and removing unimportant weights from a trained network until a given stop condition is reached. Matrix decomposition uses a compact format to represent the dense weight matrix of the fully-connected layers using few parameters, preserving the expressive power of the layer \cite{Novikov2015}. {\color{red} Matrix/tensor factorization~\cite{Denton_2014}, which exploit the linear structure of networks~\cite{Denil_2013}, or vector quantization of weights~\cite{Wu_2015} are other strategies to reduce the network memory size.} These methods reduce the amount of memory necessary to accommodate the network parameters (e.g. sharing the weights). However, they keep the same architecture, therefore requiring the same buffers (RAM) and throughput (\ac{MIPS}). Besides, network pruning requires manual setup of sensitivity for each layer and fine-tuning of the parameters.

{\color{red} A further way to achieve model compression is to reduce the weight representation to very few bits. For example, BinaryConnect~\cite{Courbariaux_2015} and the related Binary Weight Net~\cite{Rastegari_2016} represent weights with only 2 bits. If properly trained, the quantized networks can achieve performance close to the floating-point original models also on complex classification tasks~\cite{Leng_2018}. However, the memory and computational cost reductions are not sufficient for an implementation on IoT devices where few KB are available (going from 32 to 2 bits results in compression factor 16 in the memory footprint). Experiments in~\cite{Leng_2018}, in fact, do not address the low-cost low-power devices we are targeting here. In addition non-conventional frameworks are needed to train the quantized network.}
%
%\ac{SED} solutions on IoT nodes is an emerging topic. \cite{cramer2019look} describes a methodology to train embedding through self-supervised learning of audio-visual correspondence in videos, naming the resulting network L$^3$. Then Kumari et Al. \cite{kumariedgel} compress this neural network to target small edge devices, such as "motes" that use microcontrollers and achieve long-life self-powered operation. The work investigates merging of different compression techniques and highlights the increase of performance using fine-tuning after compression. 
%

 {\color{red} An attractive approach is to compress networks into a different and simpler architecture via \ac{KD} %, that transfers the knowledge of a complex model into a simpler one
\cite{buciluǎ2006model}. This approach is also referred to as Student-Teacher, because the smaller network (student) is trained to mimic the output of the larger one (teacher) \cite{shen2016teacher}.
The underlying idea is that the output of the neural network (soft labels) is richer in information than the hard labels and makes the training easier \cite{hinton2015distilling}.} {\color{red} An example of network compression related to~\ac{SED} is \cite{kumariedgel}. Starting from the L$^3$ network for embedding extraction trained through self-supervised learning of audio-visual correspondence in videos~\cite{cramer2019look}, Kumari et al. compress this neural network to target small edge devices, such as "motes" that use microcontrollers and achieve long-life self-powered operation. The work investigates merging of different compression techniques (pruning,~\ac{KD}) and highlights the increase of performance using fine-tuning after compression. }

{\color{red} Our proposed approach differentiates itself from those available in literature in multiple directions since it attempts to pull together the benefits of the methods reported above. We start from a large model and compress it. But, instead of just focusing on pruning or weight sharing, which provide limited memory reduction without decreasing the processing time, we design a very small target network and use knowledge distillation to train it (instead of training from scratch as in~\cite{Sainat2015cnnkws,Tang2018residual,zhang2017hello}). Note that distillation is typically employed to obtain small network reductions while in this paper we target extremely high compression factors. On top of this heavy compression, we apply a stochastic weight and buffer quantization without the need for retraining the network.}

%QUI FORSE CI VORREBBE UNA SORTA DI CONCLUSIONE, del tipo.
%The overview provided in this section shows the scientific interest in bringing intelligence to the edge in application domain such as computer vision and audio processing, the challenges connected and some of the possible approaches that can be followed. Our work is positioned in this broad research field, focusing on~\ac{SED}. To the best of our knowledge, this is the first attempt to use a student-teacher approach to perform sound event recognition directly on an IoT end-node with less than X mem footprint and Y processing capabilities... qualcosa del genere ma prima andrebbe verificato che non ci sono altri lavori che lo fanno.
%NON SO... forse mi sto perdendo.



==> results.tex <==
\section{Results}
\label{sec:results}
In this section, we analyze how different compression factors impact on the final classification accuracy, using the 4 losses described in Sec.\ref{sec:knowledgedistillation} and the 4 models in Table \ref{tab:models}. Figure \ref{fig:accuracyVsTraining} reports the results in terms of classification accuracy without (left) and with (right) data augmentation. First of all, the training strategy $T_{h,s,e}$ is the best performing for all model sizes. As expected, the worst approach is training the student from scratch using the hard labels ($T_{h}$). Without data augmentation, all methods are below the baseline. This is quite unexpected as the larger model is, basically, a copy of the teacher. One of the possible reasons is that \textit{UrbanSound8k} is not rich enough to learn how to mimic the VGGish model trained on a much larger dataset. This is partially confirmed in the right part of Figure~\ref{fig:accuracyVsTraining}, where data augmentation is employed: all models and training strategies substantially improve and the baseline is outperformed also by model M$_{2M}$. Note also that although the smallest network M$_{20k}$ never achieves the baseline result, its accuracy is just 5 points lower than VGGish (74.7\% vs 69.7\%) using less than 0.0424\% of the parameter and 0.12\% of the operation.  
%Approximately each line has a growing profile. It means that increasing the number of parameters always improve performance. The four lines are always one above the other. The line below is the standard back propagation training using the dataset label. It always perform worse with respect to other techniques that use hints from the teacher neural network. Slightly above the standard approach, there is the trial to copy the VGGish without using the classification output. There is always an improvement between this approach and the previous one.
%Training using the output of teacher model also gives an improvement for all models, and the gain of performance is improved when the embedded cost function \ref{eq:emb} is added to the overall cost function. 

%In the left plot, all the four lines in figure \ref{fig:accuracyVsTraining} are below the baseline. We expected that at least the biggest model achieves the baseline, but it is one point of accuracy below. The reason below this is the lack of data for our system to mimic the VGGish, that was trained on a different and bigger dataset. On the right plot there are results using data augmentation to overcome the problem. Right plot of figure \ref{fig:accuracyVsTraining} shows the results when data augmentation is employed. For all the training procedure, data augmentation improves the accuracy score. The cumbersome model overcomes the teacher baseline of around 2 accuracy point when trained with the combination of the three losses. The smallest network never achieves the baseline result, but the performance are just 5 accuracy point less (74.7\% against 69.7\%) using less than 0.0424\% of the parameter and in 0.12\% of the operation.  

\subsection{Hardware Comparison}
Since our goal is running \ac{SED} on an IoT platform, this section explores achievable performance for the set of embedded devices in Table \ref{tab:platformIntro}.
%In this section we describe network requirements versus embedded platform performance. 
For simplicity, we assume that the number of operations is equal to the number of instructions. Even if this is not true in general, the number of instructions per second is the closest number to operations per second available in microcontroller datasheets. Branch instructions are not taken into account, thus instructions are typically slightly more than operations. At the same time, most of 32 bit microcontrollers support \ac{SIMD} (multiple sums and multiplications in a single instruction), thus operations can be less than instructions. Therefore, we can assume that these two effects are balanced and the number of operation is equal to the number of instruction.
To ensure real time classification, we assume that the system must process each 960 ms audio frame (\ti1 second) before the next frame. Thus, classification time must be shorter than 1 second. Of course, we are not considering the time and resources required for other processing stages (e.g., mel-bins extraction) %This constrain is relaxed with respect to the real one, because extracting the mel-bins requires some amount of processing.
Given this two assumptions, the \ac{IPS} available should be larger or equal than the operation needed in one forward propagation. 
Memory constraints are also relevant: the RAM on-board must contain the intermediate values and the non-volatile memory should contains all network parameters. 
%We analyze performance of embedded platform in table \ref{tab:platformIntro}. For this selection, 
However, non-volatile memory is not the main limit in our examples: whenever the network does not fit in Flash memory it does not respect one of the others two parameters (RAM or \ac{IPS}). For this reason, Figure \ref{fig:availablePlatform} reports only these two constraints.

\begin{figure}[hbt]
  \centering
  \includegraphics[width=\linewidth]{ppt_available_platform.png}
  \caption{Models requirements versus hardware capabilities. Rectangles define the network requirements %: if the platform is inside the rectangle, the respective model requirements are satisfied, 
  in term of Instruction per Second (IPS) and volatile memory (RAM).}
  \label{fig:availablePlatform}
\end{figure}

None of the models proposed fits Arduino platform due to its limited RAM.
Uc32 is faster than the STM32 and TI platforms, but it cannot run the smallest model M$_{20k}$ because it would need \ti \SI{2}{\kilo\byte} of RAM more. BeagleBone Black has enough hardware capability to run most of the models, but VGGish fits only in Raspberrypi 3 B+. However, they both consumes too much. To conclude, M$_{20k}$ and M$_{200k}$ are the only suitable models for the target application. 

